Gradient Primal-Dual Algorithm Converges to Second-Order Stationary Solutions for Nonconvex Distributed Optimization

In this work, we study two first-order primal-dual based algorithms, the Gradient Primal-Dual Algorithm (GPDA) and the Gradient Alternating Direction Method of Multipliers (GADMM), for solving a class of linearly constrained non-convex optimization problems. We show that with random initialization of the primal and dual variables, both algorithms are able to compute second-order stationary solutions (ss2) with probability one. This is the first result showing that primal-dual algorithm is capable of finding ss2 when only using first-order information, it also extends the existing results for first-order, but primal-only algorithms. An important implication of our result is that it also gives rise to the first global convergence result to the ss2, for two classes of unconstrained distributed non-convex learning problems over multi-agent networks.

==> algorithm.tex <==
%!TEX root = ./boosting.tex

\vspace{-0.15in}
\section{Computational Algorithm} \label{section:algo}
\vspace{-0.1in}

Our proposed algorithm contains three nested loops: (1) homotopy optimization scheme, (2) active set strategy, and (3) minimization within active coordinates. %Details of our middle/inner loop and the discussion on advantages of our approach over PICASSO will be provided in the following sections.

\vspace{0.05in}

\noindent\textbf{(I) Outer Loop}: The homotopy optimization scheme adopts a geometrically decreasing sequence of regularization parameters $\{\lambda_t\}_{t=0}^N$ with a decay ratio $\alpha \in (0, 1)$, i.e., $\lambda_t = \alpha^t \lambda_0$. Specifically, we choose $\lambda_0=\norm{\nabla \cL(0)}_\infty$. By verifying the KKT condition, $$\min_{\xi\in\partial \cR_{\lambda_0}(0)}\norm{\nabla\cL(0)+\xi}_{\infty} = 0,$$ we have $\hat{\theta}^{\{0\}}=0$ as the optimum to \eqref{general-loss} for $\lambda=\lambda_0$. For $t\geq 1$, we initialize the solution for the $t$-th outer loop using the output solution $\hat{\theta}^{\{t-1\}}$ of the $(t-1)$-th outer loop. 
%which is used to distinguish from the optimal solution $\tilde{\theta}^{\{t\}}$, satisfying
%\begin{align*}
%\nabla\cL(\tilde{\theta}^{\{t\}})+ \xi = 0~\text{with}~\xi\in\partial \cR_{\lambda_{t}}(\tilde{\theta}^{\{t\}}),
%\end{align*}
%for solving \eqref{general-loss} with the regularization parameter $\lambda_{t}$. 
This is also known as \textit{pathwise optimization scheme}.%\citep{friedman2007pathwise,xiao2013proximal,wang2014optimal,zhao2014pathwise}.

\vspace{0.05in}

\noindent\textbf{(II) Middle Loop}: The active set identification iteratively updates the active set. Specifically, at the $k$-th iteration of the middle loop, we denote the solution by $\theta^{(k)}$, the active set containing the indices of all active coordinates by $\cA_{k}$, and denote the inactive set by $\Ac_{k} = [d] \backslash \cA_{k}$. For notional simplicity, we omit the outer loop index $t$. We update the solution by
\begin{align}
\theta^{[k+1]} = \argmin_{\theta \in \RR^d}~\cF_{\lambda} (\theta) ~~\textrm{subject to}~~\theta_{\Ac_k} = 0. \label{eqn:inner}
\end{align}
The subroutine for solving \eqref{eqn:inner} will be introduced later (inner loop). We then update the active set by the sequential screening rule. Particularly, we first shrink the active set by removing coordinates with zero values (a.k.a. the backward step),
\begin{align*}
\cA_{k+0.5} = \cA_{k}\setminus\{j\in\cA_k|&\theta_j^{[k+1]}=0\},~~\Ac_{k+0.5} = [d] \backslash \cA_{k};
\end{align*}
Then we expand the active set by adding inactive coordinates (a.k.a. the forward step),
\begin{align*}
\cA_{k+1} = \cA_{k}\cup\{j\in\Ac_{k+0.5}|~|\nabla_j\cL(\theta^{[k+1]})|\geq (1-\zeta)\lambda\},
\end{align*}
and $\Ac_{k+1} = [d] \backslash \cA_{k+1}$. As can be seen from, an inactive coordinate is selected only when its coordinate gradient of the loss function is sufficiently large in magnitude. The middle loop is terminated when the active set no longer changes. An illustrative example is provided in Figure \ref{active-set}.

\begin{figure}[H]
\vspace{-0.05in}
	\centering
	\includegraphics[width=0.475\textwidth]{Forward_Backward.pdf}
	%\vspace{-0.05in}
	\caption{\small An illustrative of the active set strategy. The active set is iteratively shrunken and expanded. Such a behavior is very similar to stepwise variable selection in classical statistics.}
	\label{active-set}
	\vspace{-0.05in}
\end{figure}

\begin{remark}
As can be seen, our proposed sequential screening rule has a explicit global control of coordinate selection based on the magnitude of the coordinate gradients of the loss function. Compared with the cyclic rule in \cite{friedman2007pathwise}, this prevents from overselection of active coordinates.  Compared with the greedy rule used in PICASSO
\begin{align*}
\cA_{k+1} = \cA_{k}\cup\{j\in\Ac_{k+0.5}|j = \argmax_j|\nabla_j\cL(\theta^{[k+1]})|\},
\end{align*}
our propose sequential screening rule can aggressively select multiple coordinates.
\end{remark}

\vspace{0.05in}

\noindent\textbf{(III) Inner Loop}:  Recall that we need to solve the subproblem \eqref{eqn:inner} in each iteration of the middle loop. Since all coordinates in $\cA_k$ stay at zero values, for notational simplicity, we rewrite \eqref{eqn:inner} as
\begin{align}\label{general-loss-active}
\tilde{\beta}^{[k+1]} = \argmin_{\beta \in \RR^s}~\tilde{\cF}_{\lambda} (\beta),
\end{align}
where $s = |\cA_k|$, $\tilde{\beta}^{[k+1]} = \theta^{[k+1]}_{\cA_k}$, $\theta^{[k+1]}_{\Ac_k} = 0$, and $\tilde{\cF}(\beta)$ denotes the same function as $\cF_{\lambda}(\theta)$ by only considering $\beta$ as the input. Similar notation applies to $\tilde{\cL}(\theta)$ and $\tilde{\ell}_i(\theta)$.

We then show how we apply use the proximal subsampled Newton algorithm to \eqref{general-loss-active} in the inner loop. For notational simplicity again, we omit the index of the middle loop for notational simplicity. Specifically, at the $m$-th iteration of the inner loop, we take
\begin{align}\label{subproblem-quadratic}
\beta^{(m+0.5)} = \argmin_{\beta \in \RR^s}\cQ(\beta;\beta^{(m)}) +  \cR_{\lambda} (\beta),
\end{align}
where $\cQ(\beta;\beta^{(m)})$ denotes the second order Tayler approximation of $\tilde{\cL}(\beta)$ at $\beta^{(m)}$, i.e.,
\begin{align}\label{quadratic-subsampled}
&\cQ(\beta;\beta^{(m)}) = \tilde{\cL}(\beta^{(m)}) + \nabla\tilde{\cL}(\beta^{(m)})^\top(\beta-\beta^{(m)})\notag\\
&\hspace{1in} + \frac{1}{2}\norm{\beta-\beta^{(m)}}_{H^{(m)}}^2.
\end{align}
Note that $H^{(m)}$ in \eqref{quadratic-subsampled} is the subsampled Hessian matrix, i.e., given $\cI_m$ sampled from $[d]$ uniformly at random,
\begin{align*}
H^{(m)} = \frac{1}{|\cI_m|}\sum_{i\in\cI_m} \nabla^2\tilde{\ell}_i(\beta^{(m)}).
\end{align*}
Compared with the exact Hessian matrix, the subsampled Hessian matrix can significantly reduce the computational cost, when $n\gg |\cI_m|$.  Once we get $\beta^{(m+0.5)}$,  we take
\begin{align*}
\beta^{(m+1)} = \beta^{(m)}+\eta_m(\beta^{(m+0.5)}-\beta^{(m)}),
\end{align*}
where $\eta$ is obtained by the backtracking line search to ensure the monotone decreasing.

\begin{remark}
Note that \eqref{subproblem-quadratic} is a regularized quadratic program, which can be efficiently solved by coordinate descent algorithms. See more details in \cite{li2016faster}.
\end{remark}


%\begin{algorithm}[t]
%\caption{Active-Set Sub-Sampled Proximal Newton (ASP-Newton) Algorithm} \label{algorithm:ASI}
%\begin{algorithmic}[1]
%\INPUT Regularization parameter $\lambda$, Initial solution $\theta^{(0)}$
%\PARAMETER Screening parameter $\zeta \in (0,0.1)$. Convergence parameter $\delta \in (0, 0.1)$
%\OUTPUT  $\hat{\theta} \leftarrow \text{ASP-Newton}(\cL, \lambda, \theta^{(0)})$.
%\State  $\cA_0 \leftarrow \{j \;|\; \theta_j^{(0)} =0, \; |\nabla_j \cL(\theta^{(0)})  |\geq (1-\zeta)\lambda \}$
%\State $\cA_0 \leftarrow \cA_0  \cup \{ j  \;\;|\;\; \theta_j^{(0)} \neq 0\}$,  $k \leftarrow 0$.
%\While {$ \min\limits _{\xi \in \partial \| \theta^{(m)} \|_1} \| \nabla \cL(\theta^{(k)}) + \lambda \xi \|_{\infty} > \delta \lambda$}
%\State $m \leftarrow 0$, $\theta^{(k, 0)} \leftarrow \theta^{(k)}$
%\While {$ \min\limits_{\xi \in \partial \| \theta^{(k,m)} \|_1 }\max\limits_{j \in \cA_k} |\nabla_j \cL(\theta^{(k,m)}) + \lambda \xi_j | > \delta \lambda$}
%\State $h_{m} \leftarrow$ solving LASSO problem \eqref{RLS} on $\cA_k$.
%\State $\theta^{(k,m+1)} \leftarrow \text{LineSearch}(\theta^{(k,m)}, h^{(m)})$ as  \eqref{linesearch}
%\State $m \leftarrow m+1$
%\EndWhile
%\State $\theta^{(k+1)} \leftarrow \theta^{(k, m)}$, $k \leftarrow k+1$.
%\State $\cA_{k+0.5} \leftarrow  \big\{ j \in \cA_k\;|\; \theta_j^{(k+1)} \neq 0 \big \}$  \Comment{Shrinkage Step}
%\State $\cA_{k+1} \leftarrow \cA_{k+0.5} \cup \big\{j~|j\in\Ac_{k}, |\nabla_j\cL(\theta^{(k+1)})|\geq(1-\zeta)\lambda \big\}$  \Comment{Expansion Step}
%\EndWhile 
%\State $\hat{\theta} \leftarrow \theta^{(k)}$.
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}[t]
%	\caption{PICASSO+SS+Newton Algorithm} \label{algorithm:ASI}
%	\begin{algorithmic}[1]
%		\INPUT Regularization parameter $\{\lambda_t \}_{t=1}^N$, Initial solution $\hat{\theta}^{\{0\}}$, Screening parameter $\zeta \in (0,0.1)$. Convergence parameter $\delta \in (0, 0.1)$
%		%\OUTPUT  $\hat{\theta} \leftarrow \text{ASP-Newton}(\cL, \lambda, \theta^{(0)})$.
%		\FOR {$t=1,\ldots,N$}
%		\STATE $\theta^{(0)} = \hat{\theta}^{\{t-1\}}$
%		\STATE  $\cA_0 \leftarrow \{j \;|\; \theta_j^{(0)} =0, \; |\nabla_j \cL(\theta^{(0)})  |\geq (1-\zeta)\lambda_t \}$
%		\STATE $\cA_0 \leftarrow \cA_0  \cup \{ j  \;\;|\;\; \theta_j^{(0)} \neq 0\}$,  $k \leftarrow 0$.
%		\WHILE {$ \min\limits _{\xi \in \partial \cR_{\lambda_t} (\theta^{(k)})} \| \nabla \cL(\theta^{(k)}) + \xi \|_{\infty} > \delta \lambda_t$}
%		\STATE $m \leftarrow 0$, $\theta^{(k, 0)} \leftarrow \theta^{(k)}$
%		\WHILE {$ \min\limits_{\xi \in \partial \cR_{\lambda_t} (\theta^{(k,m)}) }\max\limits_{j \in \cA_k} |\nabla_j \cL(\theta^{(k,m)}) + \xi_j | > \delta \lambda_t$}
%		\STATE $h_{m} \leftarrow$ solve \eqref{RLS} on $\cA_k$.
%		\STATE $\theta^{(k,m+1)} \leftarrow \text{LineSearch}(\theta^{(k,m)}, h^{(m)})$ as  \eqref{linesearch}
%		\STATE $m \leftarrow m+1$
%		\ENDWHILE
%		\STATE $\theta^{(k+1)} \leftarrow \theta^{(k, m)}$
%		\STATE $\cA_{k+0.5} \leftarrow  \big\{ j \in \cA_k\;|\; \theta_j^{(k+1)} \neq 0 \big \}$  \COMMENT{Shrinkage Step}
%		\STATE $\cA_{k+1} \leftarrow \cA_{k+0.5} \cup \big\{j~|j\in\Ac_{k}, |\nabla_j\cL(\theta^{(k+1)})|\geq(1-\zeta)\lambda_t \big\}$  \COMMENT{Expansion Step}
%		\STATE $k \leftarrow k+1$
%		\ENDWHILE 
%		\STATE $\hat{\theta}^{\{t\}} \leftarrow \theta^{(k)}$.
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm}
%
%\begin{figure}
%\centering
%\caption{An illustration of the active-set update in our algorithm. The Shrinkage and Expansion scheme ensures that the active-sets $\cA_k (k=1,2,\ldots)$ are always sparse.} \label{fig:demo}
%\includegraphics[scale=0.4]{./graphics/ASPNewton.pdf}
%\end{figure}

%\subsection{Pathwise Optimization via Decreasing Regularization Sequence }\label{pathwise-framework}
%
%To obtain a solution path for \eqref{general-loss}, we solve \eqref{general-loss} with respect to a geometrically decreasing sequence of regularization parameters $\{\lambda_t\}_{t=0}^N$ with a common decay ratio $\alpha \in [0.96, 1)$, i.e., $\lambda_t = \alpha^t \lambda_0$. Particularly, we choose $\lambda_0=\norm{\nabla \cL(0)}_\infty$ such that $\hat{\theta}^{\{0\}}=0$ is a local optimum to \eqref{general-loss} with $\lambda_0$. The first-order optimality condition gives us
%\begin{align*}
%\min_{\xi\in\partial\norm{0}_1}\norm{\nabla\cL(0)+ \lambda_0\xi}_{\infty} = 0.
%\end{align*}
%For $t = 0,...,N-1$, the previous solution $\hat{\theta}^{\{t\}}$ serves as a good warm start and we call ASP-Newton to solve
%\begin{align}\label{path-sub-loss}
%\hat{\theta}^{\{t+1\}} \leftarrow \text{ASP-Newton}(\cL, \lambda_t, \hat{\theta}^{\{t\}})
%\end{align}
%using $\hat{\theta}^{\{t\}}$ as the initial solution.


